Forgery Blind Inspection for Detecting Manipulations of Gel Electrophoresis Images

Recently, falsified images have been found in papers involved in research misconducts. However, although there have been many image forgery detection methods, none of them was designed for molecular-biological experiment images. In this paper, we proposed a fast blind inquiry method, named FBI$_{GEL}$, for integrity of images obtained from two common sorts of molecular experiments, i.e., western blot (WB) and polymerase chain reaction (PCR). Based on an optimized pseudo-background capable of highlighting local residues, FBI$_{GEL}$ can reveal traceable vestiges suggesting inappropriate local modifications on WB/PCR images. Additionally, because the optimized pseudo-background is derived according to a closed-form solution, FBI$_{GEL}$ is computationally efficient and thus suitable for large scale inquiry tasks for WB/PCR image integrity. We applied FBI$_{GEL}$ on several papers questioned by the public on \textbf{PUBPEER}, and our results show that figures of those papers indeed contain doubtful unnatural patterns.

==> Jsec02_review.tex <==
%The most common post-processing operation of WB/PCR imagery is cloning, i.e., copy-paste. Hence, although there have been several categories of image forgery detection methods \cite{farid2009image,birajdar2013digital,qazi2013survey,pun2015image}, only branches of copy-move forgery detector and feature-based methods, such as \cite{christlein2012evaluation,pun2015image,zandi2016iterative} and \cite{li2017image}, are related to this issue. However, because a user can always copy a WB/PCR band from one experiment result and paste it onto another, it is challenging to discriminate whether an unseen WB/PCR band is a clone or not. Moreover, even if two bands are suspected to be clones of the same thing due to a high PSNR value between them\footnote{Take Figure \ref{fig:exp02}(c) for example. By using block matching, the PSNR between the $2^{nd}$ band and the $6^{th}$ band can be measured as 23.8123dB, and the PSNR between the $3^{rd}$ and the $7^{th}$ bands is 22.0764dB.}, it is still not sufficient to rule out the possibility that these two bands are just similar to each other. Consequently, by assuming each scanning/photoing procedure have its own noise pattern, we deem that inappropriate post-processing operations would hopefully leave some invisible vestiges or \textit{unnatural patterns}, such as discontinuity or rectangular-boundary in the background noise, on a modified image. Consequently, the proposed fast brutal inspection method was designed to reveal unnatural patterns, indicating concealed modifications, on a WB or a PCR result. 



%The set of image forensic tools can be roughly grouped into five categories: 1) pixel-based techniques that detect statistical anomalies introduced at the pixel level; 2) format-based techniques that leverage the statistical correlations introduced by a specific lossy compression scheme; 3) camera-based techniques that exploit artifacts introduced by the camera lens, sensor, or on-chip postprocessing; 4) physically based techniques that explicitly model and detect anomalies in the three-dimensional interaction between physical objects, light, and the camera; and 5) geometric-based techniques that make measurements of objects in the world and their positions relative to the camera.

%To the best of our knowledge, we are the first to develop a fast inspection algorithm on man-made unnatural patterns on molecular-biological experiment images. Although 
Research integrity is the most essential thing in our research community. 
In order to deter tampering with experiment images, the Office of Research Integrity of U.S. already provided a photoshop-based macro, named \textit{Droplets} \cite{droplets}, for screening falsified WB/PCR images. However, because \textit{Droplets} operates based on only histogram equalization, gradient map and pseudo-coloring, it will fail to reveal features if i) the inspector sets inappropriate parameters, or ii) the brightness of a falsified WB/PCR image was carefully adjusted. Hence, \textit{Droplets} cannot be effective enough. 

Revealing invisible unnatural patterns on WB/PCR image is conceptually similar to detecting %mura defect \footnote{
``mura defect'' that describes the uneven patches of changes in luminance on thin-film-transistor liquid-crystal display (TFT-LCD) panels. %} on a TFT-LCD panels. 
However, most mura detectors were designed to identity defect regions, in which brightness is slightly different from the low-contrast background. Mura detection methods, such as \cite{watson2007spatial,shao2009robust,watson2005standard,watson2000visual,lee2004automatic,taniguchi2006mura}, would be severely disturbed by foreground bands of WB/PCR images and thus not suitable for WB/PCR forgery detection. 


Therefore, we developed our FBI$_\mbox{\tiny{GEL}}$ in a very conservative way by i) following the common idea of pseudo-background estimation used in mura defector design, and ii) exploiting a classical concept, named Hodrick-Prescott (HP) filter \cite{hpfilter1997}, in Macroeconomics. 
%for separating the volatility term from an estimated background trend of a 1D time series. 
%Note that t
The HP filter was developed to separate 
permanent shocks $\tau_t$, i.e., the stationary component or the trend component, of a 1D data series, which depicts a business cycle, from the temporary shocks $c_t = y_t - \tau_t$ causing volatility, i.e., the non-stationary part or cyclic component. %As described in Eq. \ref{eq01:HP}, given an input 1D series $y_t$, HP-filter estimates the trend component $\tau_t$ of $y_t$ via an optimization equation, and then the cyclic component can be defined as $c_t = y_t - \tau_t$.
%Briefly, the concept of HP filter can be described as below
The concept of HP filter can be summarized as below
\begin{equation}
\min_{\tau_t} \Sigma^T_{t=1}(y_t-\tau_t)^2 + \lambda \Sigma^{T-1}_{t=2} 
[ (\tau_{t+1} - \tau_t) - (\tau_t - \tau_{t-1}) ]^2 \mbox{.} % \bigg)
\label{eq01:HP}
\end{equation}


%\subsection{Hodrick-Presott Filter}
%\label{subsec:HP}

%It is generally assumed by macroeconomists that the real business cycle is induced by the interaction between \textit{permanent} shocks and \textit{temporary} shocks. Permanent shocks may result in the stationary component, also known as trend component, of a 1D data series, whereas temporary shocks cause volatility, also known as the non-stationary part or cyclic component. To separate trend component from the input data series, the Hodrick-Presott (HP) filter \cite{hpfilter1997} is one of the best known methods. Given an input 1D series $y_t$, its trend component $\tau_t$ can be derived by HP filter according to 
%\begin{equation}
%\min_{\tau_t} \Sigma^T_{t=1}(y_t-\tau_t)^2 + \lambda %\Sigma^{T-1}_{t=2} 
%[ (\tau_{t+1} - \tau_t) - (\tau_t - \tau_{t-1}) ]^2 \mbox{;} % \bigg)
%\label{eq01:HP}
%\end{equation}
%and, the cyclic component of $y_t$ is thus defined to be $c_t = y_t - \tau_t$.

%\subsection{temp}
%--------------------------------------------------------------
%
%To the best of our knowledge, we are the first to develop a fast inspection algorithm on man-made unnatural patterns on molecular-biological experiment images. Although The Office of Research Integrity of US already provide a photoshop-based macro, named Droplets \cite{droplets}, for screening counterfeit images, Droplets is a parameter-dependent method requiring user-intervention 

%
%
%希望可以利用基本的影像處理和信號處理的機制，建立一個可以快速檢驗是否有可疑殘跡的演算法，來協助整個society或是各期刊的editorial office來進行初檢工作。
%我們很確定，迄今沒有任何一個可針對分子生物學影像快速偵檢機制。雖然美國的The officie of research integrity提供了 droplets (https://ori.hhs.gov/droplets)這個工具來提供造假影像的輔助檢查，但是Droplets本身只是個photoshop-based action file (該怎麼說是一個巨集?)因此在操縱上需仰賴人為的參數調整，然而，這樣的做法會有的疑慮是，我們該如何界定某個參數所得到的圖形才可信?這樣的機制又是否對常見的壓縮方法具一定的robustness?


%--------------------------------------------------------------


\subsection{Copy-Move Detection}
\label{subsec:cpmove}
Review some TIFS papers about copy-move detection here.

\subsection{Noise Pattern Discrimination}
\label{subsec:noisechecker}
Review methods based on noise-pattern.

\subsection{Anomaly Detection}
\label{subsec:anomaly}
Is there anything related to anomaly detection?


==> Jsec03_method.tex <==

%As described in Section \ref{sec:intro}, local and manual 

%Manual modifications may still leave invisible unnatural patterns on molecular-biological images. As demonstrated in Section \ref{sec:exp}, these special patterns may include but not limited to, for example, discontinuities in the residue part and heterogeneously distributed noises \textbf{and rectangular noise regions}. 
%
%
%Our goal is here to make these invisible unnatural patterns recognizable as people already did in TFT-LCD mura defect \footnote{``Mura defect'' describes the uneven patches of changes in luminance on thin-film-transistor liquid-crystal display (TFT-LCD) panels.} detection problems \cite{watson2007spatial,shao2009robust,watson2005standard,watson2000visual,lee2004automatic,taniguchi2006mura}. 
%%One of the commonest approaches of mura detection is to measure the JND value (just noticeable difference). Because of every pixel on an image
%
%To achieve this goal, we adopt the idea of Hodrick-Presott decomposition, a very classical tool in macroeconomics, to separate the trend component from an input molecular-biological image, and then we enhance the residual to highlight unnatural patterns caused by man-made modifications.





%\subsection{Fast blind inspection on molecular-biological image}
%\label{subsec:ours}

Similar to mura detection methods designed for low-contrast images, the proposed method needs to extract an estimated pseudo-background from an input WB/PCR image first. 
%Hence, we extend the typical HP-filter to the 2D case. 
Inspired by a general idea of extracting trend and volatility components within a 1-dimensional time series, we use the optimization equation shown in Eq. (\ref{eq02:HP2d}) to define a pseudo-background $\mathcal{J}$ of an input image $\mathcal{I}$.
%
That is, 
\begin{equation}
\min_\mathcal{J} \parallel \mathcal{I}-\mathcal{J} \parallel^2_F + \lambda \parallel h * \mathcal{J} \parallel ^2_F 
\mbox{,}
\label{eq02:HP2d}
\end{equation}
where $h$ denotes a high pass kernel.
This equation forces the to-be-estimated trend component $\mathcal{J}$ to be a smoothened approximation of $\mathcal{I}$. Obviously, when $\mathcal{J}$ and $\mathcal{I}$ be images of dimension $M \times 1$ and $h=[1,-2,1]$, Eq. (\ref{eq02:HP2d}) degenerates to the 1D Hodrick-Prescott filter described in Eq. (\ref{eq01:HP}). 

However, one primary concern, in biologists' points of view, in this blind inspection problem is whether the solution can be deterministic. %\textbf{In biologists' points of view, a stochastic approach is not so appropriate since the randomness makes it difficult for the investigation committee to role-out possible chance coincidences.} 
Any randomness in the optimization solver may make it difficult for the investigation committee to role-out possible chance coincidences.
%the solution itself doubtful, although the solution converged already mathematically. 
Hence, a closed-form solution of Eq.(\ref{eq02:HP2d}) is required. To find the closed-form solution, we rewrote first Eq. (\ref{eq02:HP2d}) %we first rewrite the cost function 
by replacing Frobenius norm by matrix trace. That is, 
\begin{eqnarray}
\mathcal{L} &=& 
\parallel \mathcal{I}-\mathcal{J} \parallel^2_F + \lambda \parallel h * \mathcal{J} \parallel ^2_F \nonumber \\
&=& tr \{ (\mathcal{I}-\mathcal{J}) (\mathcal{I}-\mathcal{J})^t \} %\nonumber \\ 
%&&
+ tr\{ H \mathcal{J} H^t H \mathcal{J}^t H \}
\mbox{,}
\label{eq03:derivesol}
\end{eqnarray}
where $H$ is the Toeplitz matrix of a 1D $k$-tap-long high-pass filter $f_{k \times 1}$. That is, $h$ is now assumed to be separable and $h=f\, f^t$, where ``$t$'' denotes matrix transpose.
%
Then, letting the partial derivative of $\mathcal{L}$ with respect to $\mathcal{J}$ be zero, we obtain
\begin{eqnarray}
\frac{\partial}{\partial \mathcal{J}}\mathcal{L} %&=& 0 \nonumber \\
&=& 2 \mathcal{J}^t - 2 \mathcal{I}^t + 2 \lambda (H^t H \mathcal{J}^t H^t H)=0 \mbox{.}
\label{eq04:derivesol}
\end{eqnarray}
Therefore, we have 
\begin{equation}
\mathcal{I} = \mathcal{J} + \lambda (H^t H \mathcal{J} H^t H) \mbox{.}
\label{eq05a:solsrc}
\end{equation}
This equation guarantees that the input image $\mathcal{I}$ can be expressed as a weighting sum of a low-passed component $\mathcal{J}$ and a high-passed term $H^t H \mathcal{J} H^t H$.

%\begin{equation}
%\mathcal{I} = \mathcal{J} + \lambda (H_l H_r)^t \mathcal{J} (H_l H_r)
%\label{eq05b:solsrc}
%\end{equation}
Because $H \mathcal{J} H^t$ denotes the matrix multiplication form of a 2D  convolution $h*\mathcal{J}$, Eq. (\ref{eq05a:solsrc}) can be rewritten as 
\begin{equation}
\mathcal{I} = \mathcal{J} + \lambda ( h^t * (h* \mathcal{J}) )
\mbox{.}
\label{eq05c:solsrc}
\end{equation}
Consequently, by using discrete Fourier transform, the closed-form solution of $\mathcal{J}$ can be derived as %shown in Eq. (\ref{eq06:sol}).
\begin{equation}
\mathcal{J} = \mathcal{F}^{-1} \left \{
\frac{\mathcal{F}\{\mathcal{I}\}}
{  \mathbf{[1]} + \lambda \mathcal{F}\{h^t \} \circ \mathcal{F}\{h\} }  
\right \} \mbox{,}
\label{eq06:sol}
\end{equation}
where $\circ$ denotes Hadamard product, and $\mathbf{[1]}$ is a constant matrix whose entries are all 1's.
%With the aid of the pseudo-background $\mathcal{J}$, the volatility pattern $\mathcal{V}$ of the input image $\mathcal{I}$ can be defined as the absolute difference between $\mathcal{I}$ and $\mathcal{J}$, i.e., $\mathcal{V}=| \mathcal{I}-\mathcal{J} |$. Based on $\mathcal{V}$, the vestige of man-made modifications can be revealed. 
Based on $\mathcal{J}$, the residue pattern $\mathcal{E}$ of the input image $\mathcal{I}$ is defined to be the absolute difference between $\mathcal{I}$ and $\mathcal{J}$, i.e., $\mathcal{E}=| \mathcal{I}-\mathcal{J} |$. Based on $\mathcal{E}$, the vestige of man-made modifications can be revealed. 


%To check if there exist any unusual pattern, we first bring all pixel values of $\mathcal{V}$ into the range $[0, 1]$ and then apply hard thresholding on normalized $\mathcal{V}$ with a user-specified threshold value. Empirically, $\lambda$ in Eq. (\ref{eq06:sol}) is set to be $0.00005$, and any value in between $0.01$ and $0.5$ can be a good enough user-specified threshold.

%Such volatility pattern $\mathcal{V}$ is what we use to check if there exists any unusual pattern on the input source WB images. 

%to be $\mathcal{I}$; $| \cdot |$ denotes absolute value. 
%Consequently, the noise pattern of input image $\mathcal{I}$ is 


%----------------------------------------------------
\subsection{Selecting A High-pass Filter $h$}
\label{subsec:301}

Although $h$ was assumed to be separable whiling deriving the closed-form solution, this constraint can be relaxed in practice. Based on the concept described by Eq.(\ref{eq05c:solsrc}) that the input image $\mathcal{I}$ is a linear combination of a low-passed component $\mathcal{J}$ and a high-passed term $h^t * (h* \mathcal{J})$ extracted from $\mathcal{J}$, any high-pass filter $h$, no matter it is separable or not, can result in an optimal pseudo-background $\mathcal{J}(h, \lambda)$. 
In practice, we set $h = \delta - f$, where $f$ is a Gaussian kernel determined by MATLAB built-in function \textbf{fspecial('gaussian', [3 3], 1.0)}. 

\textbf{The design implies that $\mathcal{J}$ approximates $h*\mathcal{I}$ in some sense. (show something.)}



%----------------------------------------------------
\subsection{Revealing Unnatural Patterns}
\label{subsec:302}

To check if there exists any unusual pattern, the obtained $\mathcal{E}$ is further processed by following steps: \\
\textbf{Step-1:} Bring all pixel values of $\mathcal{E}$ into the range $[0, 1]$ and apply hard thresholding on normalized $\mathcal{E}$ with a user-specified threshold value $\gamma$. \\
\textbf{Step-2:} Binarize the thresholded normalized $\mathcal{E}$ to obtain an indicator map $\mathcal{M}_{\lambda, \gamma}$, as examples shown in Figures \ref{fig:exp04} and \ref{fig:exp01}. \\
%(a) and (b). \\%, and (c). \\
%
%
%indicating where discontinuity happens.
%Third, an optional step, we fuse $\mathcal{M}_{\lambda, \gamma}$ and $\mathcal{I}$ via alpha blending to highlight where an unnatural pattern locates. Note that in following illustrations, $\mathcal{M}_{\lambda, \gamma}$ in order to make $\mathcal{M}_{\lambda, \gamma}$ distinguishable, 
%
%
\textbf{Step-3:} Fuse $\mathcal{M}_{\lambda, \gamma}$ and $\mathcal{I}$ via alpha blending, after staining the white area of $\mathcal{M}_{\lambda, \gamma}$ yellow, to highlight where unnatural patterns locate, as the example shown in Figure \ref{fig:exp01}(c). \\
%Empirically, $\lambda$ is set to be $0.00005$, and any value in between $0.0001$ and $0.5$ can be a good enough user-specified threshold $\gamma$.
Empirically, the default value of $\lambda$ is $0.00005$; and, the default value of $\gamma$ is $0.0001$, although any value in between $0.0001$ and $0.5$ is good for $\gamma$.



%\subsection{miscs}
%we will show a 2D generalization form of the typical HP-filter and its closed-form solution. 
%%Because the standard approach for Mura defect detection\footnote{``Mura defect'' describes the uneven patches of changes in luminance on thin-film-transistor liquid-crystal display (TFT-LCD) panels. }
%
%We use the optimization equation shown in Eq. (\ref{eq02:HP2d}) to define the trend component (or the pseudobackground) $\mathcal{J}$ of a given input image $\mathcal{I}$. % should be a smoothened approximation of it. Hence, $\mathcal{J}$ can be modeled by following optimization equation



\subsection{Memo}

We need to design one another (simple) method able to indicate whether the brightness/contrast of an image was adjusted. 
Perhaps a suitable quantitative score/measure is needed. 
